Pricing, competition and market segmentation in ride hailing

We analyse a non-cooperative strategic game among two ride-hailing platforms, each of which is modeled as a two-sided queueing system, where drivers (with a certain patience level) are assumed to arrive according to a Poisson process at a fixed rate, while the arrival process of passengers is split across the two providers based on QoS considerations. We also consider two monopolistic scenarios: (i) each platform has half the market share, and (ii) the platforms merge into a single entity, serving the entire passenger base using their combined driver resources. The key novelty of our formulation is that the total market share is fixed across the platforms. The game thus captures the competition among the platforms over market share, which is modeled using two different Quality of Service (QoS) metrics: (i) probability of driver availability, and (ii) probability that an arriving passenger takes a ride. The objective of the platforms is to maximize the profit generated from matching drivers and passengers. In each of the above settings, we analyse the equilibria associated with the game. Interestingly, under the second QoS metric, we show that for a certain range of parameters, no Nash equilibrium exists. Instead, we demonstrate a new solution concept called an equilibrium cycle. Our results highlight the interplay between competition, cooperation, passenger-side price sensitivity, and passenger/driver arrival rates.

==> removed.tex <==
\textbf{Proof of lemma $\ref{lem_mr_derivation}$:} Each platform aims to maximize the individual revenue by matching the driver-passenger pair. The fraction of time spent by the driver in the state $s_i$ over the time $T$ can be given by,
$\frac{\int_0^T \mathbbm{1}_{\{X_i(x_i) = s_i\}}ds}{T}$, where $X_i(x_i)$ denotes state of process at time $x_i$. Consider a renewal cycle where renewal points are denoted by instants when the process returns to state $s_i$. Let the length of the renewal cycle be $\tau_{s_i}$. The reward in a cycle (denoted by $R_{s_i}$) is given by the time spent in state $s_i$ during this cycle. This reward is the exit time from state $s_i$. Suppose this exit time is denoted by $\xi_{s_i}$. 


Let $q_{s_i}$ be the total rate at which any transition occurs in the system when the system is in the state $s_i$.
%{\color{blue}Isn't the part where stationary distribution is equated to long-run average coming from PASTA property?}
\begin{align*}
\pi_i(s_i) &=\lim_{T \rightarrow \infty                     }\frac{\int_0^T \mathbbm{1}_{\{X_i(x_i) = s_i\}}ds}{T} \xrightarrow{\text{RRT}} \frac{1}{\E_{s_i}(\tau_{s_i})q_{s_i}}.
\end{align*}


Here, $\E_{s_i}(\tau_{s_i}) = \frac{1}{q_{s_i}\pi_i(s_i)}$,

$R_{s_i} = \int_0^{\xi_{s_i}} 1 \ ds = \xi_{s_i}$ therefore $\E[R_{s_i}] = \E[\xi_{s_i}] = \frac{1}{q_{s_i}}$.


\subsection*{Revenue generated at platform $i$}
Platform receives no revenue when the waiting driver is not available i.e., $\niw=0$. Let the platform offers the price $\phi_i(\niw)$ when the system is in the state $s_i = (\niw, \nir)$. The matching revenue generated in the renewal cycle starting at $s_i$ is: $\phi_i(\niw) \times \Prob(\text{change is due to passenger arrival)}$.


\begin{align*}
\text{reward in cycle} &= \begin{cases} \phi_i(\niw) & \text{if change is by passenger arrival}, \\ 0 & \text{else.}
\end{cases}.
\end{align*}

Let $R_i(T) $ denote the  total revenue at platform $i$ generated in time $T=[0,t]$ due to matching. Thus,
\begin{eqnarray*}
R_i(T) &=&  \sum_{\niw = 1}^{\infty} \sum_{\nir = 0}^{\infty} R_{s_i = \{\niw, \nir\}} \\
&=& \sum_{\niw = 1}^{\infty} \sum_{\nir = 0}^{\infty} \phi(\niw)\times \Prob_{s_i}\left(\text{passenger arrival}\right) \\
& = & \sum_{\niw = 1}^{\infty} \sum_{\nir = 0}^{\infty} \phi(\niw) \frac{\lambda_i(\niw)}{q_{s_i}},
\end{eqnarray*}
Here, $\lambda_i(\niw)$ denotes the passenger arrival rate when the number of waiting drivers are $\niw$ and $R_{s_i}$ is the matching revenue generated by platform $i$ while in state $s_i$. 
Here we assume that if $\{s_i:\niw = 0\}$ then $R_{s_i} = 0$.
The expected matching revenue is:
\begin{align*}
\text{Matching Revenue} & = \lim\limits_{T \rightarrow \infty} \frac{R_i(T)}{T} , \\
&= \lim\limits_{T \rightarrow \infty}  \sum_{s_i}\frac{ R_{s_i}(T)}{T} , \\
&= \sum_{s_i}\lim\limits_{T \rightarrow \infty}\frac{   R_{s_i}(T)}{T}.
\end{align*}
{\color{red} \textbf{Interchange summation and limits?}}
Here, the long-run revenue earned by the platform $i$ in state $s_i$ is given by,
\begin{align*}
\lim\limits_{T \rightarrow \infty} \frac{R_{s_i}(T)}{T} &\xrightarrow{\text{RRT}} \frac{\E[R_{s_i}]}{\E[\tau_x]},\\ &= \frac{\phi_i(\niw) \frac{\lambda_i(\niw)}{q_{s_i}}}{\frac{1}{q_{s_i}\pi_i(s_i)}},\\
\lim\limits_{T \rightarrow \infty} \frac{R_{s_i}(T)}{T} &= \phi_i(\niw)\pi_i(s_i) \lambda_i(\niw)
\end{align*}
Therefore, expected matching profit is calculated by summing the profit for a particular driver over all the states times the probability of being in the state.
\begin{equation*}
\MR_i = \sum_{s_i: \niw \neq 0} \lim\limits_{T \rightarrow \infty} \frac{R_{s_i}(T)}{T} =  \sum_{s_i} \phi_i(\niw)\pi_i(s_i) \lambda_i
\end{equation*} 

If platform $i$ quotes the price $\phi_i(\niw)$ to the arriving passenger then only $\lambda_i(\niw) f(\phi_i(\niw))$ passenger stream will enter the system and $\lambda_i(\niw) (1 - f(\phi_i(\niw)))$ part of the passenger stream will be blocked due to price. Therefore the matching revenue earned by the platform can be given as:

\begin{equation} \label{eqn_MR_expression}
\MR_i =  \sum_{s_i: \niw \neq 0} \phi_i(\niw)\pi_i(s_i) \lambda_i f(\phi_i(\niw))
\end{equation} 












The blocking probability $\pi(0)$ of a passenger is given by,
\begin{align*}
\pi(0) &= \sum_{r = 0}^{\infty} \pi((0, r)) = C e^{\frac{e}{\nu}} \left(\frac{e^0}{0!} \right) =  \frac{1}{\sum_{n=0}^{\infty} \left[\frac{e^{n}}{\prod_{a=1}^{n}(\frac{\Lambda}{2} f(\phi) + a \beta)}\right]} \\
& \approx \begin{cases}
            1 - \frac{2e}{\Lambda f(\phi)} & \text{ if }  \left(\frac{2e}{\Lambda f(\phi)}\right) < 1, \\
            0 & \text{ else.}
        \end{cases}
\end{align*}



Next we show that $g(0) < 0$ and $g(\Lambda) > 0$. Observe that $g(0) = Q_1(0) - Q_2(\Lambda)$. From \eqref{??}, we have
%\textbf{Claim:} At $\lambda_1 = 0$, $g(0) < 0$ and at $\lambda_1 = \Lambda$, $g(\Lambda) > 0$

\vspace{-4mm}

{\small \begin{align*}
g(0) &=   \left[\sum_{n_1=0}^{\infty} \left(\frac{\eiw^{n_1}}{\prod_{a=1}^{n_1}(a \beta_1)}\right)\right]^{-1} -   \left[\sum_{n_2=0}^{\infty} \left(\frac{\eiw^{n_2}}{\prod_{a=1}^{n_2}(\Lambda f(\phi_i) + a \beta_2)}\right)\right]^{-1}.
\end{align*}}

It suffices to prove the following inequality, 
$$\sum_{n_2=0}^{\infty} \left[\frac{(\eiw)^{n_2}}{\prod_{a=1}^{n_2}(\Lambda f(\phi_i) + a \beta_2)}\right] - \sum_{n_1=0}^{\infty} \left[\frac{\eiw^{n_1}}{\prod_{a=1}^{n_1}(a \beta_1)}\right] < 0.$$ to show that $g(0) < 0$. Simplifying the term on the LHS of the above inequality, we obtain %Note that for any $\beta_i \in [0, \bar{\beta}]$, both of the series are convergent. 
%
\begin{align*}
%&\sum_{n_2=0}^{\infty} \left[\frac{(\eiw)^{n_2}}{\prod_{a=1}^{n_2}(\Lambda f(\phi_i) + a \beta_2)}\right] - \sum_{n_1=0}^{\infty} \left[\frac{(\eiw)^{n_1}}{\prod_{a=1}^{n_1}(a \beta_1)}\right] = \\
& = \sum_{n=0}^{\infty} \left[\frac{\eiw^{n}}{\prod_{a=1}^{n}(\Lambda f(\phi_i) + a \beta_2)} - \frac{\eiw^{n}}{\prod_{a=1}^{n}(a \beta_1)}\right]. \\
& = \sum_{n=0}^{\infty} \eiw^{n} \left[\frac{n!\beta_1^n - \prod_{a=1}^{n}(\Lambda f(\phi_i) + a \beta_2) }{\left(\prod_{a=1}^{n}(\Lambda f(\phi_i) + a \beta_2)\right)\left(\prod_{a=1}^{n}(a \beta_1)\right)} \right].
\end{align*}
For a given pair of $\beta_1, \beta_2$, w.l.o.g., assume that $\beta_1 \leq \beta_2$. Therefore we get
$n!\beta_1^n - \prod_{a=1}^{n}(\Lambda f(\phi_i) + a \beta_2) < 0$. If $\beta_1 > \beta_2$ then defining the function $g(\lambda_2) = Q_1(\Lambda - \lambda_2) - Q_2(\lambda_2)$ and following the above procedure, we will get $g(0) < 0$.
On similar lines, we get $g(\Lambda) = Q_1(\Lambda) - Q_2(0)$ and using similar arguments as above we get $g(\Lambda) > 0$. 

Thus, $g$ satisfies the hypothesis of Intermediate Value Theorem (IVT). Using IVT, there exists a $\lambda_1 = \lambda^* \in (0, \Lambda)$ such that $g(\lambda^*) = 0$.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\textbf{Proof of Lemma \ref{lem_pio_WE}}: %At Wardrop Equilibrium when using $\pi_i(0)$ as a WE metric, the blocking probability of the both the platforms must be same i.e., $\pi_1(0) = \pi_2(0)$. 
From Lemma \ref{lem_exist_unique_WE} we know that there exist an unique WE with $\DA_i$ as a WE metric. Our aim is to find the passenger arrival rate split  at WE $(\lambda_1, \lambda_2)$. 
 
The proof follows by contradiction. If possible, assume $\lambda_1 f(\phi_1) > \lambda_2 f(\phi_2)$  and observe $\lambda_i f(\phi_i)$ is the effective passenger arrival rate to the platform $i \in \mathcal{N}$. Here note that $\lambda_2 = \Lambda - \lambda_1$. Then from Lemma \ref{lem_Montone_with_Arrival_rate}   $N_1 \stackrel{d}{\le} N_2$, i.e., $P (N_1 \ge n) \ge  P (N_2 \ge n)$ for all $n$, where both are the two stationary probabilities. In particular $P(N_1 > 0) \ge P(N_2 > 0)$ and hence   $  \DA_1 = P(N_1=0) <  P(N_2=0) =  \DA_2$.  Thus $(\DA_2-\DA_1) > 0.$
By Lemma \ref{lem_exist_unique_WE}  $\DA_i$ is strictly monotone in $\lambda_i$. Thus one can increase $\DA_1$ and decrease $\DA_2$ by decreasing $\lambda_1$. In all, $\DA_2 - \DA_1$ is a continuous and strictly decreasing function of $\lambda_1$, which 


, which reduces the gap $(\DA_2-\DA_1)^2$, contradicting the definition of WE. 


, which is a contradiction to the definition of WE, which requires $\DA_1 = \DA_2$. 
One can give similar arguments for the case when $\lambda_1 f(\phi_1) < \lambda_2 f(\phi_2)$. 

Thus at WE, the split must be such that $\lambda_1 f(\phi_1) = \lambda_2 f(\phi_2)$. Simplifying it further (using $\lambda_2 = \Lambda - \lambda_1$), we obtain the following: \begin{eqnarray}
%\lambda_1 f(\phi_1) &=& (\Lambda - \lambda_1) f(\phi_2), \nonumber \\
\lamo = \frac{\Lambda f(\phi_2)}{f(\phi_1) + f(\phi_2)} \text{ and } \lamt = \frac{\Lambda f(\phi_1)}{f(\phi_1) + f(\phi_2)}. \nonumber \hspace{10mm}
\text{\eop}
\end{eqnarray}  






\section{Analysis for $f(\phi) = 1 - \frac{\phi}{\phi_h + \epsilon}$}
\begin{enumerate}
\item $\phimr := {\arg \max}_{\phi \in [0, \phi_h]} \{\Lambda f(\phi) \phi - e\phi\}$
    
$m(\phi) = \Lambda f(\phi) \phi - e\phi.$ By differentiating the function $m$, we get $m'(\phi) = \Lambda - e -  \Lambda \frac{2 \phi}{\phi_h + \epsilon}$. By equating $m'(\phi) = 0$, we get $ \phimr = \frac{\Lambda - e}{2\Lambda}(\phi_h + \epsilon) = \left(\frac{1 - x}{2} (\phi_h + \epsilon) \right)$.  Since $m''( \phimr) < 0$, $\phimr$ is maximizer of the function $m$.
    
    
\item $\phifp := {\arg \max}_{\phi \in [0, \phi_h]} \{f(\phi) \phi\}$
    
Let $\P(\phi) = f(\phi) \phi$. By differentiating the function $\P$, we get $\P'(\phi) = 1 - \frac{{2\phi}}{\phi_h + \epsilon}$. By equating $\P'(\phi) = 0$, we get $\phifp = \frac{\phi_h + \epsilon}{2}$. Since $\P'(\phifp) < 0$, $\phifp$ is maximizer of the function $\P$.

    
\item $\phibar = f^{-1}\left( \frac{e}{\Lambda}\right) \implies f(\phibar) =  \frac{e}{\Lambda} \implies 1 - \frac{\phibar}{\phi_h + \epsilon} =  \frac{e}{\Lambda} \\ \therefore \phibar = \left( 1 - \frac{e}{\Lambda}\right)(\phi_h + \epsilon) $.
    
    
\item $\phiunderbar = f^{-1}\left( \frac{2e}{\Lambda}\right)\implies f(\phiunderbar) =  \frac{2e}{\Lambda} \implies 1 - \frac{\phiunderbar}{\phi_h + \epsilon} =  \frac{2e}{\Lambda} \\ \therefore \phiunderbar = \left( 1 - \frac{2e}{\Lambda}\right)(\phi_h + \epsilon) $. (possible only if $\Lambda > 3e$)

\item $\eL = \frac{\mstar}{e} = \frac{m(\eU)}{e} = \frac{(\Lambda - e)^2}{4e\Lambda}(\phi_h + \epsilon) = \frac{(\phi_h + \epsilon)}{4}\left( \frac{1}{x} -2 + x\right)$.
\item $\phido = \frac{2 (\phi_h + \epsilon)}{3}$ 

$d(\phido) = 2 - \frac{3\phido}{\phi_h}$
\end{enumerate}



\section{Analysis for $f(\phi) = 1 - \sqrt{\frac{\phi}{\phi_h + \epsilon}}$}
\begin{enumerate}
    \item $\phimr := {\arg \max}_{\phi \in [0, \phi_h]} \{\Lambda f(\phi) \phi - e\phi\}$
    
    Let $g_1(\phi) = \Lambda f(\phi) \phi - e\phi.$ Therefore $g_1(\phimr) = \Lambda \phimr - \Lambda \phimr \sqrt{\frac{\phimr}{\phi_h + \epsilon}} - e\phimr$. Taking derivative of the function $g_1$ and equating it to zero, we get $g_1'(\phimr) = \Lambda - e -  \frac{3\Lambda}{2} \sqrt{\frac{ \phimr}{\phi_h + \epsilon}} = 0$
    
    $\therefore \phimr = \left(\frac{2(\Lambda - e)}{3\Lambda}\right)^2(\phi_h + \epsilon) = \frac{4}{9}(1 - x)^2 (\phi_h + \epsilon)$
    
    
    \item $\phifp := {\arg \max}_{\phi \in [0, \phi_h]} \{\Lambda f(\phi) \phi\}$
    
    Let $g_2(\phi) = \Lambda f(\phi) \phi.$ Therefore $g_2(\phifp) = \Lambda \phifp - \Lambda \phifp \sqrt{\frac{\phifp}{\phi_h + \epsilon}}$. Taking derivative of the function $g_2$ and equating it to zero, we get $g_2'(\phifp) = \Lambda -   \frac{3\Lambda}{2} \sqrt{\frac{ \phifp}{\phi_h + \epsilon}} = 0$
    
    $\therefore \phifp = \frac{4}{9}(\phi_h + \epsilon)$
    
    
    \item $\phibar = f^{-1}\left( \frac{e}{\Lambda}\right) \implies f(\phibar) =  \frac{e}{\Lambda} \implies 1 - \sqrt{\frac{\phibar}{\phi_h + \epsilon}} =  \frac{e}{\Lambda} \\ \therefore \phibar = \left( 1 - \frac{e}{\Lambda}\right)^2 (\phi_h + \epsilon) $.
    
    
    \item $\phiunderbar = f^{-1}\left( \frac{2e}{\Lambda}\right)\implies f(\phiunderbar) =  \frac{2e}{\Lambda} \implies 1 - \sqrt{\frac{\phiunderbar}{\phi_h + \epsilon}} =  \frac{2e}{\Lambda} \\ \therefore \phiunderbar = \left( 1 - \frac{2e}{\Lambda}\right)^2 (\phi_h + \epsilon) $.
    
    \item $\eL = \frac{\mstar}{e} = \frac{m(\eU)}{e} = \frac{4(\Lambda - e)^3}{27e\Lambda^2}(\phi_h + \epsilon) = \frac{4}{27} (\phi_h + \epsilon) \left( \frac{1}{x} - x^2 - 3 + 3x\right)  $.
    \item $\phido = \frac{16 (\phi_h + \epsilon)}{25}$
\end{enumerate}


\subsection{Simulation - NE for $\beta \approx 0 \ \ \& \ \ \beta > 0 $ are matching}



\



\ignore{\begin{equation}
\DAl_i = \begin{cases}
    1 - \frac{\eiw}{\lami f(\phi_i)} & \text{ if }  \left(\frac{\eiw}{\lami f(\phi_i)}\right) < 1, \\
           0 & \text{ else.}
   \end{cases} 
\end{equation}}

Limit system ($\bbeta=0$)
W.l.o.g. when $\phi_1>\phi_2$,
\begin{equation}
    WE_1 = \begin{cases}
  \lamo   & \text{ if } \frac{e}{(\lami f(\phi_i))}<1 \text{ for } i= \{1,2\} \\
  \lamo & \text{ if } \frac{e}{\lami f(\phi_i)}\ge 1 \text{ for } i= \{1,2\} 
    \end{cases}
\end{equation}
We proved WE is continuous in $\bbeta$ for all $\bbeta > 0$. Then the following limits exist:
$$
\lambda_i^*(\VPhi) := \lim_{ \bbeta \to (0,0) } \lami  
$$

At WE we have for any $\bbeta > 0$ (only stability is required, which is always true when $\bbeta > 0$ )
$$
\lambda_1 f(\phi_1) = \lambda_2 f(\phi_2)  
$$
Therefore WE split does not depend upon $\bbeta$ and hence easy to define
$$
\lambda_i^*(\VPhi) :=   \lami  
$$

Thus WE of limit system coincides with limit of the WE (when the first condition in (8) is true)
